Flexibility of Integrated Power and Gas Systems: Gas Flow Modeling and Solution Choices Matter

Due to their slow gas flow dynamics, natural gas pipelines function as short-term storage, the so-called linepack. By efficiently utilizing linepack, the natural gas system can provide flexibility to the power system through the flexible operation of gas-fired power plants. This requires accurately representing the gas flow physics governed by partial differential equations. Although several modeling and solution choices have been proposed in the literature, their impact on the flexibility provision of gas networks to power systems has not been thoroughly analyzed and compared. This paper bridges this gap by first developing a unified framework. We harmonize existing approaches and demonstrate their derivation from and application to the partial differential equations. Secondly, based on the proposed framework, we numerically analyze the implications of various modeling and solution choices on the flexibility provision from gas networks to power systems. One key conclusion is that relaxation-based approaches allow charging and discharging the linepack at physically infeasible high rates, ultimately overestimating the flexibility.

==> 10_Pu_conversion.tex <==
% First approaches by xx and yy to apply a normalization ...
% But those distort the solution of the problem as they ar enot obyeing the units or choosing too many base values.
% %Approaches distort the solution
% Another suggestion in \cite{Herty2009} seems appealing from numerical perspective but slightly distorts the solution of the original problem. It further requires a constant diameter of all pipelines in the network, which is a rather restrictive assumption that is hardly met in practise.
% In contrast to existing approaches in the literature, we propose a per unit conversion which is mathematically equivalent to the original problem and does not impose any assumptions on the network topology.

\section{Applying per unit conversion} \label{section:pu}
Due to the slow dynamics of gas flows in pipelines, the OPGF is numerically challenging. Taking a look at the conservation of momentum constraint~\eqref{eq:momentum_d} in the main paper, assuming a pipeline diameter $D = 1\,\unit{\meter}$ and space discretization of $\Delta x = 50\,\unit{\kilo\meter}$, the coefficients in front of the pressure drop and friction factor are around $10^{-4}$ and $10^{4}$, respectively. Note that refining the discretization reduces the numerical issues.

Similar to power systems analysis, those numerical issues can be tackled by applying a per-unit conversion, which transforms all variables and parameters into dimensionless quantities without distorting the underlying relations and the structure of the problem. This is done by defining interdependent base values according to the physical dimensions of the variables and parameters.

For the PDEs governing the gas flow, there are three degrees of freedom in choosing the bases. We decide to choose a base for the pressure $\Pi^{\mathrm{B}}$ in $\unit{\pascal}$, the spatial dimension $D^{\mathrm{B}}$ in $\unit{\meter}$ and time $T^{\mathrm{B}}$ in $\unit{\second}$. From those, the bases for the cross-sectional area $A^{\mathrm{B}}$ in $\unit{\meter\squared}$, the speed of sound in gas $C^{\mathrm{B}}$ in $\unit{\meter\per\second}$, and the one for the mass flow $M^{\mathrm{B}}$ in $\unit{\kilo\gram\per\second}$ are derived based on their respective units:
\begin{align}\label{eq:bases_def}
    A^{\mathrm{B}} = (D^{\mathrm{B}})^2, \quad C^{\mathrm{B}} = D^{\mathrm{B}}/T^{\mathrm{B}}, \quad M^{\mathrm{B}} = D^{\mathrm{B}} \Pi^{\mathrm{B}} T^{\mathrm{B}}.
\end{align}

The bases for the auxiliary variable $\gamma$, $\Gamma^{\mathrm{B}}$ is derived based on Equation~\eqref{eq:gamma_def} in the main paper as:
\begin{equation}\label{eq:gamma_base_def}
    \Gamma^{\mathrm{B}} = \frac{(M^{\mathrm{B}})^2}{\Pi^{\mathrm{B}}}.
\end{equation}

All model parameters are then divided by their respective bases. The solution to the original problem can be recovered by multiplying the optimal solutions of the decision variables by their respective bases. As long as the bases are derived according to the physical dimensions, the problems with and without per-unit conversion are mathematically equivalent.%\footnote{Due to numerical issues, the solutions of the original problem and the converted problem slightly differ in practice.}

GFPPs couple the power and gas systems based on their gas-to-power conversion efficiency $\eta$ in \unit{\mega\watt\per\kilo\gram\second}. Using the base power $S^{\mathrm{B}}$ of the power system, the base value for the efficiency can be calculated as $\eta^{\mathrm{B}} = M^{\mathrm{B}}/S^{\mathrm{B}}$. This makes the proposed per-unit conversion for the gas system appealing to integrated power and gas system studies, as it is widely established in power systems analysis.

For this study we choose $\Pi^{\mathrm{B}} = \mathrm{\qty{1}{\mega\pascal}}$, $D^{\mathrm{B}} = \mathrm{\qty{1}{\meter}}$, and $T^{\mathrm{B}} = \mathrm{\qty{1}{\second}}$. The remaining base values can be calculated as explained above. %Note that the range of the parameters, i.e., the optimal value of problem~\eqref{eq:optimal_pu_base}, decreases with a finer discretization, such that the numerical issues are reduced.
Note that refining the discretization reduces the numerical issues.
Finally, we transform all the cost parameters of the objective function using a cost base of \qty{1000}{\eur}.

% To apply the per-unit conversion to different gas networks and discretizations and avoid a manual tuning of base values, we solve a small unconstrained minimization problem to find the optimal bases for spatial and time dimensions $D^{\mathrm{B}}$ and $T^{\mathrm{B}}$, respectively, which minimizes the Euclidean distance between the magnitudes of the parameters of the conservation of mass and momentum constraints~\eqref{eq:mass_d}--\eqref{eq:momentum_d} and a center $Z$:
% \begin{align}
% \begin{split}\label{eq:optimal_pu_base}
%     \min_{D^{\mathrm{B}},T^{\mathrm{B}}} & (\log_{10} \left( \frac{T^{\mathrm{B}}}{\Delta t} \right) - Z)^2 + (\log_{10} \left( \frac{(c \cdot T^{\mathrm{B}})^2 D^{\mathrm{B}}}{\Delta x} \right) - Z)^2 + \\
%     & (\log_{10} \left( \frac{T^{\mathrm{B}}}{\Delta t} \right) - Z)^2 + (\log_{10} \left( \frac{1}{D^{\mathrm{B}} \Delta x} \right) - Z)^2 + (\log_{10} \left( \frac{\widetilde{\lambda} (c \cdot T^{\mathrm{B}})^2 D^{\mathrm{B}}}{2 \widetilde{D}^3 \Delta x} \right) - Z)^2,
% \end{split}
% \end{align}
% where $\Delta x$ and $\Delta t$ are the chosen space and time discretization, $c$ is the speed of sound in the gas, and $\widetilde{\lambda}$ and $\widetilde{D}$ are the friction factor and the pipeline diameter that reflect the network topology. We choose the average friction factor and smallest pipeline diameter observed in the network. Based on feasibility tolerances of $10^{-4}$, we choose $Z = 1$.

% For high-pressure gas transmission networks, we choose $\Pi^{\mathrm{B}} = 0.5\,\unit{\mega\pascal}$. Based on problem~\eqref{eq:optimal_pu_base}, we find values of around $ D^{\mathrm{B}} = 1 \cdot 10^{-7}$ and $D^{\mathrm{T}} = 2 \cdot 10^3$ for a discretization of $\Delta t = 1\,\unit{\hour}$ and $ D^{\mathrm{B}} = 2.5 \cdot 10^{-7}$ and $D^{\mathrm{T}} = 1 \cdot 10^3$ for $\Delta t = 15\,\unit{\minute}$. The remaining base values can be calculated as explained above. Note that the range of the parameters, i.e., the optimal value of problem~\eqref{eq:optimal_pu_base}, decreases with a finer discretization, such that the numerical issues are reduced.

==> 11_Nomenclature.tex <==
Naming convention:
Gas
	- Set of gas nodes I,j in I
	- Set of pipes (I,j) in P
	- Gas flow m
	- Set of gas sources S
	- Set of gas demands D
 	- Gas supply and demand: q
  	- Flow direction binary decision variable: z
	- Set of compressors C
    - Nodal gas pressure variable: $\pi$
    - superscript for curtailment? $q^{\mathrm{O}}_{t,d}$ O? or we re-use D?
 Power
 	- Set of power buses n,m in N
	- Set of dispatchable generators K
	- Set of gas fired G \subseteq K
 	- Set of wind power plants W
	- Set of power demands R
	- Set of lines (n,m) in L
	- Power flow f
	- Power supply and demand: p


==> Impact_modeling.tex <==

\section{Gas flow problem: Impact of modeling choices} 
\label{section:03_modelcomp}
In this section, we assess the impact of modeling choices on the optimal gas flow problem. Similarly to \cite{ConorThesis}, we do not take a power system perspective but focus on gas network state variables. Therefore, we do not solve the integrated optimal power-gas flow problem, but only the optimal gas flow problem. This consists in minimizing objective function (25) without power system costs, subject to the gas system constraints (28a)-(29). A stylized 3-node natural gas transmission network is used as an illustrative case study. The network topology is shown in Figure \ref{fig_1}, and all the parameters are reported in the Github repository \cite{Online_Companion}. The simplifying assumptions introduced to obtain the $\mathrm{ST}$ and $\mathrm{QD}$ models are challenged when the gas load changes rapidly (i.e., the temporal derivatives in \eqref{eq:mass}-\eqref{eq:momentum} give a significant contribution). Therefore, we analyze an extreme scenario where the gas load at node 2 is linearly increased from 10\% to 100\% over 30 minutes, representing, for instance, the sudden ramp-up of a very large gas-fired peak power plant. Considering an efficiency of 30\% and a gas lower heating value of 13.6 kWh/kg, the power plant size is 1469 MW. The load at node 3 is kept constant during the 5-hour time horizon. Before the ramp-up starts at hour 3:00, the cheaper gas source S1 is able to cover both loads. The more expensive source S2 (which could for example represent a large underground storage facility) is activated to meet the increasing load, resulting in a change of flow direction for pipeline 2. The load input data are provided every 5 minutes, and the optimization problem is solved with the open-source nonlinear solver Ipopt. 

\begin{figure}
\centering
\includegraphics[width=2.5in]{Pictures/gas_network_3nodes.png}
\caption{Schematic representation of the 3-node natural gas network.}
\label{fig_1}
\end{figure}

\subsection{Impact of discretization}
First, the impact of space and time discretization is analyzed. For the $\mathrm{ST}$ model, having a more refined discretization in space does not give an additional contribution, since the mass flow is assumed to be constant along the pipe, as explained in Section \ref{subsection:02_steadystate}. Having a more refined discretization in time gives a contribution only if the load input data are available with a granularity smaller than the chosen time step (e.g., the load data are available every 15 minutes, and a 1-hour time step is adopted). By choosing a coarser discretization (e.g., 1-hour) and performing the average, the peaks in the load profile are smoothed out. However, if the load input data are provided only every hour, refining the time discretization and assuming that the load is constant over the whole hour does not affect the solution of the steady-state model. 

Conversely, for the $\mathrm{QD}$ and $\mathrm{DY}$ models, we observe that the space and time discretization have a significant impact on the optimal solution since they directly affect the way the original PDEs are approximated. This is often neglected in the literature about integrated power-gas systems, where generally a 1-hour time step and no space discretization (i.e., in each pipeline, $\Delta x$ equal to its length) are adopted \cite{Correa-Posada2015, ZENG2017, He_ADMM_2017, ORDOUDIS2019, Qadrdan2014}, without assessing the solution quality. We focus here on the QD model, but the presented results similarly apply to the DY model. The solution obtained with our most refined discretization in space and time chosen here, $\Delta x = 5$ km and $\Delta t = 300$ s, is used as a reference to compare the impact of a coarser mesh. 

In Fig. \ref{fig_disc_space}, the impact of space discretization on the pressure values at node 3 is shown: $\Delta x$ is gradually increased by keeping $\Delta t $ constant and equal to the reference. For $\Delta x = 100$ km, equal to the length of the pipelines, a maximum relative error of -4.9\% with respect to the reference is observed. By only discretizing each pipeline in two segments (i.e., $\Delta x = 50$ km) the maximum relative error is reduced to -0.8\%. Similarly, in Fig. \ref{fig_disc_time}, the impact of time discretization is assessed. By choosing a 1-hour time-step, a maximum relative error of 13.1\% is observed, while with 15 minutes, this is significantly reduced to 1.4\%. Improving the temporal discretization has a bigger impact on the solution accuracy than improving the spatial discretization. The reason is that the finite difference method used to discretize the original PDEs is characterized by a first order error in time, and second order error in space (i.e., the error decreases linearly with $\Delta t$ and quadratically with $\Delta x$) \cite{ConorThesis,helgaker2013}. Finally, in Fig. \ref{fig_disc_both}, the combined impact of both space and time discretizations is assessed, comparing the most refined reference discretization, with an intermediate discretization ($\Delta x = 50$ km and $\Delta t = 900$ s), and the very coarse discretization that is often adopted in the literature (1-hour time discretization, and no space discretization). In Fig. \ref{fig_2}, the pressure at node 3 is used to illustrate the impact of discretization, but significant relative errors are observed also on the values of the other optimal variables, such as pipeline inflow and outflow, dispatch decisions, and linepack estimation. The latter especially is critical when assessing the flexibility provided by the natural gas network to the power system. Since the linepack value is proportional to the average pressure in the pipe, as shown by \eqref{eq:lp}, a significant error in the pressure at the nodes can result in an overestimation or underestimation of the linepack potential. In the analyzed case study, the relative error on the linepack value of pipeline 2 reaches 8.6\% in one of the time instants when the most coarse discretization is adopted (1-hour time discretization, and no space discretization), and only 0.8\% if we choose the intermediate discretization ($\Delta x = 50$ km and $\Delta t = 900$ s). The discretization, especially the temporal one, should therefore be carefully selected when modeling the integrated operation of the power-gas system to avoid an overestimation of linepack flexibility. The day-ahead scheduling for power systems is generally solved with a 1-hour time step, but using the same discretization for the gas problem could lead to significant errors in the flexibility estimation. 
%A finer discretization improves the solution quality but negatively impacts the computational time needed to solve the problem. The three solutions in Fig. \ref{fig_disc_both}, are obtained respectively in 186, 6.1, and 5.5 seconds (from finer to coarser discretization). The intermediate discretization proposed represents a satisfactory compromise between solution accuracy and computational effort. It has to be noted, however, that the computational time is relatively high for such a small case gas network. The efficient solution of an approximated quasi-dynamic model will be further addressed in Section \ref{section:04_NGsol}.

\begin{figure*}[!h]
\centering
\subfloat[]{\includegraphics[width=2.1in]{Pictures/pressure3_space_stairs.png}%
\label{fig_disc_space}}
\hfil
\subfloat[]{\includegraphics[width=2.1in]{Pictures/pressure3_time_stairs.png}%
\label{fig_disc_time}}
\hfil
\subfloat[]{\includegraphics[width=2.1in]{Pictures/pressure3_both_stairs.png}%
\label{fig_disc_both}}
\caption{Pressure at node 3 for the quasi-dynamic model. (a) Impact of space discretization. (b) Impact of time discretization. (c) Combined impact of space and time discretization.}
\label{fig_2}
\end{figure*}

\subsection{$\mathrm{DY}$ vs. $\mathrm{QD}$ vs. $\mathrm{ST}$}
The $\mathrm{ST}$ model is not suitable to assess the flexibility provided by the gas network to the power system since it does not capture linepack flexibility. Moreover, adopting the $\mathrm{ST}$ model for describing the short-term operation of natural gas networks can lead to infeasible and sub-optimal solutions for real-time operation. We hypothesize that the $\mathrm{ST}$ model could be adequate for long-term planning problems, but the error introduced by neglecting the linepack on the investment decisions should be further assessed and is out of the scope of this paper. %The $\mathrm{ST}$ model is solved significantly faster than the other two models (for the most refined discretization, the computational time is reduced by around 98\% and 97\% with respect to the $\mathrm{QD}$ and $\mathrm{DY}$ models, respectively). 
It has to be reminded that, for the $\mathrm{ST}$ model, refining the spacial discretization does not improve the solution accuracy, therefore $\Delta x$ equal to the length of the pipeline is always adopted in this analysis. Fig. \ref{fig_3} shows the pressure profile at node 3 for the $\mathrm{ST}$, $\mathrm{QD}$ and $\mathrm{DY}$ models with our most refined discretization. Since the $\mathrm{QD}$ and $\mathrm{DY}$ profile overlap almost perfectly, the right y-axis of Fig. \ref{fig_3} shows the relative error between the two models (considering the $\mathrm{DY}$ model as a reference). For all time-steps, the relative error is lower than 0.1\%. The relative error is even lower if a coarser time discretization is adopted. 

\begin{figure}[!t]
\centering
\includegraphics[width=3.4 in]{Pictures/pressure3_QD_D.png}
\caption{Left axis: pressure at node 3 for the steady-state ($\Delta x = 100$ km and $\Delta t = 300$), quasi-dynamic ($\Delta x = 5$ km and $\Delta t = 300$), and dynamic model ($\Delta x = 5$ km and $\Delta t = 300$). Right axis: relative error between the quasi-dynamic and dynamic model.}
\label{fig_3}
\end{figure}

As already highlighted in Section \ref{subsection:02_quasidynamic}, the QD model is obtained by neglecting the inertia term (i.e., the temporal derivative) in the momentum equation. By rearranging \eqref{eq:momentum_d}, we express the pressure drop in each pipeline (or sub-pipeline) as \cite{Hennings2021}:
\begin{align}
    &\pi_{i,t}-\pi_{j,t} = \underbrace{\frac{\Delta x}{A}\frac{m_{ij,t}-m_{ij,t-1}}{\Delta t}}_\text{$\alpha$} + \underbrace{\frac{\Delta x}{A}\frac{\lambda c^2}{2DA}\frac{m_{ij,t}|m_{ij,t}|}{\pi_{ij,t}}}_\text{$\beta$},  \label{eq:alpha}
\end{align}
where $\alpha$ represents the contribution of the inertia term to the total pressure drop, and $\beta$ is the contribution of the friction with the inner pipeline walls. Since the pressure drop is the sum of the inertia and friction contributions, the $\mathrm{QD}$ model is a satisfactory approximation of the $\mathrm{DY}$ model when the value of $\alpha$ is small (in both absolute and relative terms). In realistic operating conditions, the inertia term can be considered negligible when $|\alpha| < \SI{50}{Pa/km}$ and $|\alpha|/|\beta| < 1\%$  \cite{Hennings2021}.

In our case study, due to the very fast ramp up of the load in node 2, the thresholds are shortly exceeded in pipeline 2, where the change in flow direction occurs. This is shown is Fig. \ref{fig_4}, where the pressure drop contributions are plotted from hour 3:00 to hour 4:30. The plot inset in Fig. \ref{fig_4} depicts the absolute and relative contribution of $\alpha$ in pipeline 2 compared to the defined thresholds. During the fast ramp up, the thresholds are both violated during only 5 time-steps (out of 60). When the flow approaches zero (before changing direction) and $\beta$ is almost zero, the relative contribution of $\alpha$ is not negligible, but the absolute threshold is not violated. In pipeline 1, despite the very fast ramp-up occurring, both the absolute and relative thresholds for $\alpha$ are never violated. 

\begin{figure}[!t]
\centering
\includegraphics[width=3 in]{Pictures/alpha_D.png}
\caption{Pressure drop in pipeline 2 from hour 3:00 to hour 4.30: contribution of the inertia and friction terms. The inset plot shows the absolute and relative contribution of the inertia term in pipeline 2 compared to the defined thresholds.}
\label{fig_4}
\end{figure}
Even in the very extreme case study considered, the thresholds are only shortly violated. If a bigger discretization time-step is selected, the impact of the inertia term would be even smaller. In accordance with what is found in \cite{Hennings2021, Osiadacz1984, Herran2009}, the $\mathrm{QD}$ model is suitable to be used for the scheduling phase while the dynamic model has to be adopted in real-time to ensure feasibility (similarly to the power system, where DC OPF is used for scheduling, while AC OPF is then adopted for real-time operation). 
%However, we observe that in our case including the inertia term does not increase computational complexity when the model is solved with IPOPT. Actually, the $\mathrm{DY}$ model is solved faster than the $\mathrm{QD}$ model likely due to the reduced feasibility region. For our case study with the most refined discretization tested, the $\mathrm{DY}$ model is solved in around 130 seconds, while the $\mathrm{QD}$ in around 180 seconds. To sum up, when the problem is solved with IPOPT, the dynamic model should be preferred especially to better capture the gas dynamics without increasing the computational burden. If instead, an approximated convexified problem is solved, as will be discussed in Section \ref{section:04_NGsol}, the $\mathrm{QD}$ model should be preferred. This can be especially relevant when prices have to be derived for market applications. 
Improving the discretization (especially the time discretization) has a bigger impact on solution accuracy than including the inertia term.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tikz/large_case.tex <==

\definecolor{color_blue_1}{rgb}{0.267004,0.004874,0.329415}
\definecolor{color_blue_2}{rgb}{0.229739,0.322361,0.545706}
\definecolor{color_blue_3}{rgb}{0.128729,0.563265,0.551229}
\definecolor{color_blue_4}{rgb}{0.360741,0.785964,0.387814}
\definecolor{color_blue_5}{rgb}{0.993248,0.906157,0.143936}


\ctikzset{bipoles/length=0.85cm}

% \def\storage#1#2{
% \begin{scope}[shift={#1}, rotate=#2]
%     % \node[black, line width=0.25mm, fill = gray!50, opacity=1, regular polygon,regular polygon sides=4, draw, shape border rotate=0, scale = 2] at (0,0){};
%     \node[anchor=north west,inner sep=0] at (0,0) {
%             \includegraphics[height=1.1cm]{storage.png}};
% \end{scope}
% }


\def\legendx{0}
\def\legendy{-0.5}

\def\boxheight{0.5cm}
\def\boxwidth{1cm}   

\newcommand{\mycolorbox}[1]{
    \fill[#1] ($(\legendx,\legendy)+(0,\theboxnum*\boxheight)$) rectangle ($(\legendx,\legendy)+(\boxwidth,\theboxnum*\boxheight+\boxheight))$;
    \addtocounter{boxnum}{1}
}
\def\ticklength{0.2cm}
\newcommand{\colortick}[2]{
    \draw ($(\legendx,\legendy)+(\boxwidth,#1*\boxheight)$) -- ($(\legendx,\legendy)+(\boxwidth+\ticklength,#1*\boxheight)$);
    \node[anchor=west] at ($(\legendx,\legendy)+(\boxwidth+\ticklength, #1*\boxheight)$) {#2};
}




% Define custom shape for compressorStation
\tikzset{
    compressor/.style={
        append after command={
            \pgfextra{
                \fill[black] ($(\tikzlastnode.north west)+(-0.1,0)$) -- ($(\tikzlastnode.east)+(0.1,0.3)$) -- ($(\tikzlastnode.east)+(0.1,-0.3)$) -- ($(\tikzlastnode.south west)+(-0.1,0)$) -- cycle;
}}}}

\tikzset{
    compressor90/.style={
        append after command={
            \pgfextra{
                \fill[black] ($(\tikzlastnode.north west)+(0,0.1)$) -- ($(\tikzlastnode.south)+(-0.3,-0.1)$) -- ($(\tikzlastnode.south)+(0.3,-0.1)$) -- ($(\tikzlastnode.north east)+(0,0.1)$) -- cycle;
}}}}

\tikzset{
    compressor180/.style={
        append after command={
            \pgfextra{
                \fill[black] ($(\tikzlastnode.north east)+(0.1,0)$) -- ($(\tikzlastnode.west)+(-0.1,0.3)$) -- ($(\tikzlastnode.west)+(-0.1,-0.3)$) -- ($(\tikzlastnode.south east)+(0.1,0)$) -- cycle;
}}}}

\begin{figure}
    \centering

    \resizebox{17cm}{!}{%

     \begin{circuitikz}  %[>=triangle 45]

        \draw[thick] ($(\legendx,\legendy)+(-0.25,+0.25)$) rectangle ($(\legendx,\legendy)+(2.5,3.9)$);
        \draw ($(\legendx,\legendy)+(-0.125,3.5)$) node[anchor=west] {RMS [\%]};
        
        \fill[color_blue_1] ($(\legendx,\legendy)+(0,1*\boxheight)$) rectangle ($(\legendx,\legendy)+(\boxwidth,1*\boxheight+\boxheight))$
        \fill[color_blue_2] ($(\legendx,\legendy)+(0,2*\boxheight)$) rectangle ($(\legendx,\legendy)+(\boxwidth,2*\boxheight+\boxheight))$
        \fill[color_blue_3] ($(\legendx,\legendy)+(0,3*\boxheight)$) rectangle ($(\legendx,\legendy)+(\boxwidth,3*\boxheight+\boxheight))$
        \fill[color_blue_4] ($(\legendx,\legendy)+(0,4*\boxheight)$) rectangle ($(\legendx,\legendy)+(\boxwidth,4*\boxheight+\boxheight))$
        \fill[color_blue_5] ($(\legendx,\legendy)+(0,5*\boxheight)$) rectangle ($(\legendx,\legendy)+(\boxwidth,5*\boxheight+\boxheight))$

        \draw ($(\legendx,\legendy)+(\boxwidth,2*\boxheight)$) -- ($(\legendx,\legendy)+(\boxwidth+\ticklength,2*\boxheight)$);
        \node[anchor=west] at ($(\legendx,\legendy)+(\boxwidth+\ticklength, 2*\boxheight)$) {2.5};
        \draw ($(\legendx,\legendy)+(\boxwidth,3*\boxheight)$) -- ($(\legendx,\legendy)+(\boxwidth+\ticklength,3*\boxheight)$);
        \node[anchor=west] at ($(\legendx,\legendy)+(\boxwidth+\ticklength, 3*\boxheight)$) {5};
        \draw ($(\legendx,\legendy)+(\boxwidth,4*\boxheight)$) -- ($(\legendx,\legendy)+(\boxwidth+\ticklength,4*\boxheight)$);
        \node[anchor=west] at ($(\legendx,\legendy)+(\boxwidth+\ticklength, 4*\boxheight)$) {7.5};
        \draw ($(\legendx,\legendy)+(\boxwidth,5*\boxheight)$) -- ($(\legendx,\legendy)+(\boxwidth+\ticklength,5*\boxheight)$);
        \node[anchor=west] at ($(\legendx,\legendy)+(\boxwidth+\ticklength, 5*\boxheight)$) {10};


        \begin{scope}[shift={(2.5,-2)}]
            % Frame around the legend
            \draw[thick] (-0.5,-0.5) rectangle (28,+0.5);
        
            
            % % Legend title
            % \draw (4,2.5) node[anchor=center] {\textbf{Legend}};

            % Gas system
            \draw (0,0) node[draw, regular polygon, regular polygon sides=3, inner sep=3pt] {};
            \draw (0.3,0) node[anchor=west] {Gas source};
            %
            \draw (2.8,0) node[circle, inner sep=3pt, draw] {};
            \draw (3.1,0) node[anchor=west] {Node};
            %
            \draw (5,0) node[draw, rectangle, inner sep=5pt] {};
            \draw (5.3,0) node[anchor=west] {Gas load};
            %
            \draw (8,0) node[compressor180] {};
            \draw (8.3,0) node[anchor=west] {Compressor};
            %

            \draw[thick] (11,-0.5) -- (11,+0.5);
            %Power system,
            \draw[->] (12,-0.25) -- +(0,0.5); 
            \draw (12.3,0) node[anchor=west] {Electrical load};

            % Generators
            \draw[color = black] (16,-0.25) to [sV] (16,0.25) node[]{};
            \draw (16.5,0) node[anchor=west] {Non-GFPP};
            %
            \draw[color = color_WF] (20,-0.25) to [sV] (20,0.25) node[]{};
            \draw (20.5,0) node[anchor=west] {Windgenerator};
            %
            \draw[color = color_GFPP] (24,-0.25) to [sV] (24,0.25) node[]{};
            \draw (24.5,0) node[anchor=west] {GFPP};
            %
            \draw [ultra thick] (26.3,-0.25) -- (26.3,0.25);
            \draw (26.6,0) node[anchor=west] {Bus};
            
        \end{scope}


        % Define nodes%%%%%% Gas Network
        \foreach \type/\id/\no/\labelpos/\x/\y in {
        source/source_3/1/above/6/1.25,
        innode/innode_4/2/below/7.5/1.25,
        innode/innode_5/3/above/7.5/2.5,
        sink/sink_27/4/above/9/2.5,
        sink/sink_19/5/below/9/1.25,
        innode/innode_2/6/above/10.5/1.25,
        sink/sink_10/7/below/12/1.25,
        sink/sink_11/8/below/13.5/1.25,
        innode/innode_1/9/below/15/1.25,
        sink/sink_16/10/left/15/2.5,
        sink/sink_14/11/right/12/2.5,
        sink/sink_13/12/right/12/3.75,
        innode/innode_6/13/right/12/5,
        sink/sink_25/14/above right/12/6.25,
        source/source_1/15/right/15/7.5,
        sink/sink_3/16/right above/15/6.25,
        sink/sink_23/17/left/15/5,
        innode/innode_8/18/above/13.5/6.25,
        source/source_2/19/above/9/10,
        innode/innode_7/20/above/10.5/10,
        sink/sink_29/21/right/12/10,
        sink/sink_28/22/above/12/11.25,
        sink/sink_2/23/above/13.5/8.75,
        sink/sink_15/24/left/12/7.5,
        sink/sink_20/25/below/10.5/5,
        sink/sink_4/26/below/9/6.25,
        sink/sink_8/27/above/9/3.75,
        sink/sink_17/28/below/7.5/5,
        sink/sink_5/29/below/6/5,
        sink/sink_7/30/below/4.5/5,
        sink/sink_24/31/below/3/5,
        sink/sink_21/32/below/1.5/5,
        sink/sink_12/33/below/0/5,
        sink/sink_26/34/above/9/7.5,
        sink/sink_9/35/above/7.5/7.5,
        sink/sink_18/36/above/6/7.5,
        sink/sink_6/37/above/4.5/7.5,
        sink/sink_22/38/above/2.25/7.5,
        sink/sink_1/39/above/0/7.5,
        subnode/subnode_1/40/above/11.25/1.25,
        subnode/subnode_2/41/above/11.25/5.625,
        subnode/subnode_3/42/above/12/1.875,
        subnode/subnode_4/43/above/10.5/6.875,
        subnode/subnode_5/44/above/15/1.875
        }
        {
            \ifthenelse{\equal{\type}{source}}{
                \node[draw, regular polygon, regular polygon sides=3, inner sep=3pt, label=\labelpos:\Large$i_{\no}$] (\id) at (\x,\y) {};
            }{
                \ifthenelse{\equal{\type}{innode}}{
                    \node[draw, circle, inner sep=3pt, label=\labelpos:\Large$i_{\no}$] (\id) at (\x,\y) {};
                }{
                    \ifthenelse{\equal{\type}{subnode}}{
                        \node[inner sep=0pt] (\id) at (\x,\y) {};
                    }{
                        \node[draw, rectangle, inner sep=5pt, label=\labelpos:\Large$i_{\no}$] (\id) at (\x,\y) {};
                    }
                }
            }
        }

        % \node[draw, circle, inner sep=3pt, label=\labelpos:\Large$i_{\no}$] (\id) at (\x,\y) {};
        % GFPP gas loads
        \draw[->, color=color_GFPP] (sink_16) -- +(0.75,0) node[below right] {\Large$g_1$}; 
        \draw[->, color=color_GFPP] (sink_10) -- +(0.75,-0.75) node[below right] {\Large$g_2$}; 
        \draw[->, color=color_GFPP] (sink_27) -- +(0.75,0) node[above right] {\Large$g_3$};
        \draw[->, color=color_GFPP] (sink_18) -- +(0,-0.75) node[below right] {\Large$g_{5/6}$}; 
        \draw[->, color=color_GFPP] (sink_26) -- +(0.75,0) node[above right] {\Large$g_7$}; 
        \draw[->, color=color_GFPP] (sink_2) -- +(0,-0.75) node[below right] {\Large$g_{10}$};
        \draw[->, color=color_GFPP] (sink_3) -- +(0.75,-0.75) node[below right] {\Large$g_{11/12}$}; 
    


        % pipeline connections
        \foreach \start/\stop/\pipeNo/\color in {
            innode_4/innode_5/1/color_blue_1,
            sink_27/innode_5/2/color_blue_2,
            sink_27/sink_19/3/color_blue_4,
            innode_4/sink_19/4/color_blue_5,
            sink_10/innode_2/5/color_blue_2,
            sink_10/sink_11/6/color_blue_3,
            innode_1/sink_16/7/color_blue_2,
            sink_14/sink_10/8/color_blue_1,
            sink_13/sink_14/9/color_blue_1,
            innode_6/sink_13/10/color_blue_1,
            source_1/sink_3/11/color_blue_1,
            sink_3/sink_23/12/color_blue_2,
            sink_25/innode_8/13/color_blue_2,
            sink_29/innode_7/14/color_blue_3,
            sink_29/sink_28/15/color_blue_1,
            sink_29/sink_2/16/color_blue_2,
            sink_2/sink_15/17/color_blue_3,
            sink_15/sink_29/18/color_blue_2,
            sink_25/sink_15/19/color_blue_4,
            sink_25/sink_20/20/color_blue_2,
            sink_4/sink_20/21/color_blue_1,
            sink_17/sink_4/22/color_blue_1,
            sink_8/sink_20/23/color_blue_1,
            sink_17/sink_8/24/color_blue_2,
            sink_5/sink_17/25/color_blue_1,
            sink_7/sink_5/26/color_blue_1,
            sink_6/sink_7/27/color_blue_3,
            sink_7/sink_24/28/color_blue_4,
            sink_24/sink_21/29/color_blue_3,
            sink_21/sink_12/30/color_blue_1,
            sink_25/sink_26/31/color_blue_1,
            sink_26/sink_4/32/color_blue_1,
            sink_26/sink_9/33/color_blue_1,
            sink_9/sink_18/34/color_blue_1,
            sink_18/sink_6/35/color_blue_2,
            sink_6/sink_22/36/color_blue_1,
            sink_22/sink_1/37/color_blue_1,
            subnode_1/sink_10/38/color_blue_2,
            subnode_2/sink_20/39/color_blue_2,
            subnode_3/sink_14/40/color_blue_2,
            subnode_4/sink_26/41/color_blue_1,
            subnode_5/sink_16/42/color_blue_2,
        }{
            \draw[color=\color, line width = 2.5] (\start) -- (\stop); 
        }


        % \foreach \start/\stop/\pipeNo/\color/\infnorm/\anchor in {
        %     innode_4/sink_19/4/color_blue_5/14.5/south,
        %     sink_29/innode_7/14/color_blue_3/10.6/south,
        %     sink_25/sink_15/19/color_blue_4/10.1/south,
        % }{
        %     % \draw[color=\color, line width = 2.5] (\start) -- (\stop); 
        %     \node[anchor=\anchor] (Pipe\pipeNo) at ($(\start)!0.5!(\stop)$) {\infnorm};
        % }
        
        % Compressors
        \foreach \id/\x/\y in {
            % compressorStation_2/11.25/0,
            compressorStation_6/14.25/6.25
        }{
            \node[compressor] (\id) at (\x,\y) {};
        }
        
        \foreach \id/\x/\y in {
            compressorStation_2/14.25/1.25,
            compressorStation_3/9.75/1.25, 
            compressorStation_4/6.75/1.25, 
            compressorStation_5/9.75/10
        }{
            \node[compressor180] (\id) at (\x,\y) {};
        }
        
        \foreach \id/\label/\x/\y in {
            compressorStation_1/1/12/5.6
            %compressorStation_6/6/15/5
        }{
            % \node[compressor90, label=right:\Large$c_{\label}$] (\id) at (\x,\y) {};
            \node[compressor90] (\id) at (\x,\y) {};
        }
        
        % Compressor connections
        \foreach \from/\to in {
            compressorStation_1/sink_25,
            compressorStation_1/innode_6,
            compressorStation_2/innode_1,
            compressorStation_2/sink_11,
            compressorStation_3/innode_2,
            compressorStation_3/sink_19,
            compressorStation_4/innode_4,
            compressorStation_4/source_3,
            compressorStation_5/innode_7,
            compressorStation_5/source_2,
            compressorStation_6/innode_8,
            compressorStation_6/sink_3,
        }{
            \draw[line width = 2] (\from) -- (\to);
        }


        % %%%%% Power network
        \begin{scope}[shift={(17,0)}]

            \foreach \start/\name/\direction/\rot/\shift  in {
                {2,1}/n_{1}/north west/0/{-1,0},
                {10,1}/n_{2}/north west/0/{-1,0},
                {1,4.5}/n_{3}/east/0/{1,0},       
                {3.5,3.25}/n_{4}/east/0/{0,-1},      
                {7.5,3.25}/n_{5}/east/0/{0,-1},       
                {16,3}/n_{6}/north/0/{0,1},  
                {14,1}/n_{7}/north west/0/{-1,0},
                {16,1.5}/n_{8}/north/0/{0,1},    
                {9,4.5}/n_{9}/east/0/{1,0},        
                {13,4.5}/n_{10}/east/0/{1,0},     
                {9,6.25}/n_{11}/east/0/{1,0},
                {13,6.25}/n_{12}/east/0/{1,0},
                {16,6.75}/n_{13}/north/0/{0,1},
                {5,6.25}/n_{14}/east/0/{1,0},
                {1,8}/n_{15}/south east/0/{1,0},
                {6,8}/n_{16}/west/0/{-1,0}, 
                {1,9.75}/n_{17}/east/0/{1,0},
                {5,9.75}/n_{18}/east/0/{1,0},
                {9,8}/n_{19}/east/0/{1,0}, 
                {13,8}/n_{20}/east/0/{1,0}, 
                {9,9.75}/n_{21}/east/0/{1,0},
                {13,9.75}/n_{22}/east/0/{1,0},
                {16,9.25}/n_{23}/south/0/{0,-1},
                {1,6.25}/n_{24}/north east/0/{1,0},
            } {
                \node[anchor=\direction] (\name) at (\start) {\Large$\name$};
                \draw [ultra thick] (\start) -- ($(\start)+(\shift)$);
            }
    
            % Loads
            \draw[->] (1+0.75,1) -- +(0,-0.75); %l1
            \draw[->] (9+0.75,1) -- +(0,-0.75); %l2
            \draw[->] (1+0.5,4.5) -- +(0,-0.75); %l3
            \draw[->] (3.5,2.25+0.5) -- +(0.75,0); %l4
            \draw[->] (7.5,2.25+0.5) -- +(-0.75,0); %l5
            \draw[->] (16,3+0.5) -- +(0.75,0); %l6
            \draw[->] (13+0.75,1) -- +(0,-0.75); %l7
            \draw[->] (16,1.5+0.5) -- +(0.75,0); %l8
            \draw[->] (9+0.5,4.5) -- +(0,0.75); %l9
            \draw[->] (13+0.5,4.5) -- +(0,0.75); %l10
            \draw[->] (16,6.25+0.75) -- +(0.75,0); %l13
            \draw[->] (5+0.5,6.25) -- +(0,-0.75); %l14
            \draw[->] (1+0.25,8) -- +(0,0.75); %l15
            \draw[->] (5+0.75,8) -- +(0,-0.75); %l16
            \draw[->] (5+0.75,9.75) -- +(0,+0.75); %l18
            \draw[->] (9+0.5,8) -- +(0,-0.75); %l19
            \draw[->] (13+0.5,8) -- +(0,-0.75); %l20

    
            % Network
            \draw (13.75,1) -- (13.75,1.25) -- (15.75,1.75) -- (16,1.75); %line 7-8
            \draw (16,3.25) -- (15.75,3.25) -- (9.75,1.25) -- (9.75,1);   %line 2-6
            \draw (16,3.75) -- (15.75,3.75) -- (13.75,4.25) -- (13.75,4.5); %line 6-10
            \draw (7.5,3) -- (7.75,3) -- (13.25,4.25) -- (13.25,4.5);    %line 5-10
            \draw (16,2.25) -- (15.75,2.25) -- (13.5,4.25) -- (13.5,4.5); %line 8-10
            \draw (16,2) -- (15.75,2) -- (9.75,4.25) -- (9.75,4.5);   %line 8-9
            \draw (3.5,3) -- (3.75,3) -- (9.5,4) -- (9.5,4.5);       %line 4-9
            \draw (3.5,2.5) -- (3.75,2.5) -- (9.5,1.5) -- (9.5,1);     %line 2-4
            \draw (1.75,1) -- (1.75,1.25) -- (9.25,1.25) -- (9.25,1);    %line 1-2
            \draw (1.5,1) -- (1.5,1.5) -- (7.25,2.5) -- (7.5,2.5);      %line 1-5
            \draw (1.25,4.5) -- (1.25,4.25) -- (1.25,1.5) -- (1.25,1);     %line 1-3
            \draw (1.75,4.5) -- (1.75,4.25) -- (9.25,4.25) -- (9.25,4.5);     %line 3-9
            \draw (13.25,6.25) -- (13.25,6) -- (9.75,5) -- (9.75,4.5);  %line 9-12
            \draw (13.25,4.5) -- (13.25,4.75) -- (9.75,6) -- (9.75,6.25);  %line 10-11
            \draw (13.75,4.5) -- (13.75,6.25);  %line 10-12
            \draw (9.25,4.5) -- (9.25,6.25);  %line 9-11
            \draw (1.5,4.5) -- (1.5,6.25);  %line 3-24
            \draw (1.5,8) -- (1.5,6.25);  %line 15-24
            \draw (13.75,6.25) -- (13.75,6.5) -- (15.75,7) -- (16,7);  %line 12-13
            \draw (9.75,6.25) -- (9.75,6.5) -- (15.75,7.25) -- (16,7.25);  %line 11-13
            \draw (16,7.5) -- (15.75,7.5) -- (15.75,8.5) -- (16,8.5);  %line 13-23
            \draw (13.25,6.25) -- (13.25,6.5) -- (15.75,8.75) -- (16,8.75);  %line 12-23
            \draw (13.75,8) -- (13.75,8.25) -- (15.75,9) -- (16,9);  %line 20-23
            \draw (5.75,6.25) -- (5.75,6.5) -- (9.25,6.5) -- (9.25,6.25);  %line 14-11
            \draw (5.5,8) -- (5.5,6.25);  %line 14-16
            \draw (1.75,8) -- (1.75,8.25) -- (5.25,8.25) -- (5.25,8); %line 15-16
            \draw (1.5,8) -- (1.5,8.5) -- (9.5,9) -- (9.5,9.75); %line 15-21
            \draw (1.5,9.75) -- (1.5,9.25) -- (13.75,9.25) -- (13.75,9.75);  %line 17-22
            \draw (9.75,8) -- (9.75,8.25) -- (13.25,8.25) -- (13.25,8); %line 19-20
            \draw (5.75,8) -- (5.75,8.25) -- (9.25,8.25) -- (9.25,8);  %line 16-19
            \draw (1.25,9.75) -- (1.25,9) -- (5.5,8.5) -- (5.5,8);  %line 17-16
            \draw (1.75,9.75) -- (1.75,9.5) -- (5.25,9.5) -- (5.25,9.75);  %line 17-18
            \draw (5.75,9.75) -- (5.75,9.5) -- (9.25,9.5) -- (9.25,9.75);  %line 18-21
            \draw (9.75,9.75) -- (9.75,9.5) -- (13.25,9.5) -- (13.25,9.75); %line 21-22
    
            %%% Conventional generators
            \draw[color = color_GFPP] (1.25,0.75) to [sV] (1.25,0.25) node[anchor=north east]{\Large$g_1$};
            \draw[color = color_GFPP] (1.25,1)--(1.25,0.75);
            \draw[color = color_GFPP] (9.25,0.75) to [sV] (9.25,0.25) node[anchor=north east]{\Large$g_2$};
            \draw[color = color_GFPP] (9.25,1)--(9.25,0.75);
            \draw[color = color_GFPP] (13.25,0.75) to [sV] (13.25,0.25) node[anchor=north east]{\Large$g_3$};
            \draw[color = color_GFPP] (13.25,1)--(13.25,0.75);
            \draw[color = black] (16.5,7.75) node[anchor = north west, rotate=0, xshift=10, yshift=3]{\Large $g_4$}  to [sV] (16.5,7.25) ;
            \draw[color = black] (16,7.5)--(16.25,7.5);
            \draw[color = color_GFPP] (0.75,7.75) to [sV] (0.75,7.25) node[anchor=north east, xshift=0, yshift=0]{\Large$g_{5/6}$};
            \draw[color = color_GFPP] (1.25,8)--(1.25,7.5)--(1,7.5);
            \draw[color = color_GFPP] (4.75,7.75) to [sV] (4.75,7.25) node[anchor=north east, xshift=0, yshift=0]{\Large$g_{7}$};
            \draw[color = color_GFPP] (5.25,8)--(5.25,7.5)--(5,7.5);
            \draw[color = color_GFPP] (16.5,8.75) node[anchor = north west, rotate=0, xshift=10, yshift=3]{\Large $g_{11/12}$}  to [sV] (16.5,8.25) ;
            \draw[color = color_GFPP] (16,8.5)--(16.25,8.5);
            \draw[color = black] (5.25,10.5) to [sV] (5.25,10) node[anchor=south east, yshift=12]{\Large$g_8$};
            \draw[color = black] (5.25,10)--(5.25,9.75);
            \draw[color = black] (9.25,10.5) to [sV] (9.25,10) node[anchor=south east, yshift=12]{\Large$g_9$};
            \draw[color = black] (9.25,10)--(9.25,9.75);
            \draw[color = color_GFPP] (13.25,10.5) to [sV] (13.25,10) node[anchor=south east, yshift=12]{\Large$g_{10}$};
            \draw[color = color_GFPP] (13.25,10)--(13.25,9.75);
        
        
            % %%% Wind farms
            \draw[color = color_WF] (2.25,5.25) to [sV] (2.25,4.75) node[anchor=south west, xshift=0, yshift=12]{\Large$w_{1}$};
            \draw[color = color_WF] (1.75,4.5)--(1.75,5)--(2,5);
            \draw[color = color_WF] (8,2.75) to [sV] (8,2.25) node[anchor=north west, xshift=2, yshift=0]{\Large$w_{2}$};
            \draw[color = color_WF] (7.5,2.5)--(7.75,2.5);
            \draw[color = color_WF] (13.25,1.75) to [sV] (13.25,1.25) node[anchor=south west, xshift=5, yshift=10]{\Large$w_3$};
            \draw[color = color_WF] (13.25,1)--(13.25,1.25);
            \draw[color = color_WF] (2.25,7.75) to [sV] (2.25,7.25) node[anchor=north west, xshift=0, yshift=-2]{\Large$w_{4}$};
            \draw[color = color_WF] (1.75,8)--(1.75,7.5)--(2,7.5);
            \draw[color = color_WF] (10.5,10.5) to [sV] (10.5,10) node[anchor=south west, xshift=0, yshift=12]{\Large$w_{5}$};
            \draw[color = color_WF] (9.75,9.75)--(9.75,10.25)--(10.25,10.25);
        
        \end{scope}
            
    \end{circuitikz}
    }

% \end{tikzpicture}
\caption{Case study B: GasLib 40-node gas network connected to 24-bus IEEE RTS system. Innode 3 and pipelines 33 and 39 are removed from the gas network to avoid circular flows arising from the neglect of compressor states. Pipeline colors indicate the value of the root mean squared (RMS) relaxation gap of each pipeline for the optimal solution of model $\mathrm{DY}$-$\mathrm{PELP}$.}
\label{fig:large_case}
\figspace
\end{figure}

==> tikz/small_case_3.tex <==
\ctikzset{bipoles/length=0.85cm}
\def\legendx{1}
\def\legendy{9}

\def\boxheight{0.5cm}
\def\boxwidth{1cm}   

\def\ticklength{0.2cm}
\newcommand{\colortick}[2]{
    \draw ($(\legendx,\legendy)+(\boxwidth,#1*\boxheight)$) -- ($(\legendx,\legendy)+(\boxwidth+\ticklength,#1*\boxheight)$);
    \node[anchor=west] at ($(\legendx,\legendy)+(\boxwidth+\ticklength, #1*\boxheight)$) {#2};
}

 \begin{circuitikz}[>=triangle 45]

        \begin{scope}[shift={(-1,-8)}, font=\large]
            % Frame around the legend
            \draw[thick] (-1,-0.5) rectangle (26,+0.5);

            % Gas system
            \draw (0,0) node[draw, regular polygon, regular polygon sides=3, inner sep=3pt] {};
            \draw (0.3,0) node[anchor=west] {Gas source};
            %
            \draw (3,0) node[circle, inner sep=3pt, draw] {};
            \draw (3.3,0) node[anchor=west] {Node};
            %
            \draw (5,0) node[draw, rectangle, inner sep=5pt] {};
            \draw (5.3,0) node[anchor=west] {Gas load};
            %

            \draw[thick] (8,-0.5) -- (8,+0.5);
            %Power system,
            \draw[->] (9,-0.25) -- +(0,0.5); 
            \draw (9.3,0) node[anchor=west] {Electrical load};

            % Generators
            \draw[color = black] (13,-0.25) to [sV] (13,0.25) node[]{};
            \draw (13.5,0) node[anchor=west] {Non-GFPP};
            %
            \draw[color = color_dark_blue] (17,-0.25) to [sV] (17,0.25) node[]{};
            \draw (17.5,0) node[anchor=west] {Windgenerator};
            %
            \draw[color = red] (21,-0.25) to [sV] (21,0.25) node[]{};
            \draw (21.5,0) node[anchor=west] {GFPP};
            %
            \draw [ultra thick] (24,-0.25) -- (24,0.25);
            \draw (24.5,0) node[anchor=west] {Bus};
            
        \end{scope}
        \scalebox{1.5}{  
        \begin{scope} [shift={(-1,-12)}]
    %%%%%%% Power system %%%%%%%
    % Nodes
    \draw [ultra thick] (2,9) node[anchor=south, rotate = 0]{\Large$n_{1}$} -- (2,8);
    \draw [ultra thick] (5,9) node[anchor=south, rotate = 0]{\Large$n_{2}$} -- (5,8);
    \draw [ultra thick] (3,10) node[anchor=east, rotate = 0]{\Large$n_{3}$} -- (4,10);
    % Loads
    \draw[->] (3.5,10) -- +(0,0.75); %l1
    \draw[->] (2,8.2) -- +(-0.75,0); %l2
    % Network
    \draw (2,8.2) -- (5,8.2);  %line 1-2
    \draw (2,8.8) -- (2.25,8.8) -- (3.2,9.75) -- (3.2,10);  %line 1-3
    \draw (5,8.8) -- (4.75,8.8) -- (3.8,9.75) -- (3.8,10);  %line 1-3

    %%% Conventional generators
    \draw (1.5,8.9)  to [sV] (1.5,8.4) node[anchor= north east, rotate=0, yshift = 20, xshift = -15]{\Large$g_1$}; %[anchor= north east, rotate=0, yshift = 20, xshift = -15]
        \draw (1.75,8.65)--(2,8.65);

    \draw [color = red] (5.75,9.05)  to [sV] (5.75,8.6);
    \node[rotate=0] at (6.6,8.85) {\Large$\textcolor{red}{g_2}$};
    \draw [color = red] (5,8.85)--(5.5,8.85);

    %%% Wind farms
    \draw[color = color_dark_blue] (5.75,8.45)   to [sV] (5.75,7.95); %windfarm1
    %\draw[color = color_dark_blue] (7.3,8.4)--(7.5,8.4);
    %\draw[color = color_dark_blue] plot [smooth cycle] coordinates {(7.55,8.9) (7.5,8.4) (7.45,7.9) (7.55,7.9) (7.5,8.4) (7.45,8.9) };
    \draw[color = color_dark_blue] (5,8.2)--(5.5,8.2);
    \node[rotate=0] at (6.6,8.2) {\Large$\textcolor{color_dark_blue}{w_1}$};

    %%%%%%% Gas system %%%%%%%
    \pgfmathsetmacro{\s}{0.08}
    % Nodes
    \node[draw, regular polygon, regular polygon sides=3, inner sep=3pt, label=below:\Large$i_{1}$] (i1) at (10,8.2) {};
    \node[draw, circle, inner sep=3pt, label=below:\Large$i_{2}$] (i2) at (13,8.2) {};
    \node[draw, regular polygon, regular polygon sides=3, inner sep=3pt, label=below:\Large$i_{3}$] (i3) at (15,8.2) {};
    \node[draw, rectangle, inner sep=5pt, label=right:\Large$i_{4}$] (i4) at (13,9.4) {};
    \node[circle, fill=white, inner sep=0pt] (gfpp) at (5.75, 9.4) {};
    % Pipes
    \draw (i1) -- (i2) node[midway,below] {\Large$p_{1}$};
    \draw (i2) -- (i3) node[midway,below] {\Large$p_{2}$};
    \draw (i2) -- (i4) node[midway,left] {\Large$p_{3}$};
    % Coupling
    \draw [dashed,color = red] (i4) -- (gfpp) -- (5.75, 9.05); %(12, 9) -- (12, 10.5) -- (6.9, 10.5)
    % Gas load
    %\draw[->] (i4) -- +(0,1); %l1
    \end{scope}
    }
    \end{circuitikz}
    

==> tikz/small_case_v2.tex <==
\ctikzset{bipoles/length=0.85cm}
 \begin{circuitikz}[>=triangle 45]
    %%%%%%% Power system %%%%%%%
    % Nodes
    \draw [ultra thick] (2,9) node[anchor=south, rotate = 0]{\Large$n_{1}$} -- (2,8);
    \draw [ultra thick] (5,9) node[anchor=south, rotate = 0]{\Large$n_{2}$} -- (5,8);
    \draw [ultra thick] (3,10) node[anchor=east, rotate = 0]{\Large$n_{3}$} -- (4,10);
    % Loads
    \draw[->] (3.5,10) -- +(0,0.75); %l1
    \draw[->] (2,8.2) -- +(-0.75,0); %l2
    % Network
    \draw (2,8.2) -- (5,8.2);  %line 1-2
    \draw (2,8.8) -- (2.25,8.8) -- (3.2,9.75) -- (3.2,10);  %line 1-3
    \draw (5,8.8) -- (4.75,8.8) -- (3.8,9.75) -- (3.8,10);  %line 1-3

    %%% Conventional generators
    \draw (1.5,8.9)  to [sV] (1.5,8.4) node[anchor= north east, rotate=0, yshift = 20, xshift = -15]{\Large$g_1$}; %[anchor= north east, rotate=0, yshift = 20, xshift = -15]
        \draw (1.75,8.65)--(2,8.65);

    \draw (6.9,9.7)  to [sV] (6.9,9.2) node[anchor= south, yshift = 17.5]{\Large$g_2$};
    \draw (6,9.45)--(6.65,9.45);

    %%% Wind farms
    \draw[color = color_dark_blue] (6.9,8.7)   to [sV] (6.9,8.2); %windfarm1
    %\draw[color = color_dark_blue] (7.3,8.4)--(7.5,8.4);
    %\draw[color = color_dark_blue] plot [smooth cycle] coordinates {(7.55,8.9) (7.5,8.4) (7.45,7.9) (7.55,7.9) (7.5,8.4) (7.45,8.9) };
    \draw[color = color_dark_blue] (6,8.45)--(6.65,8.45);
    \node[rotate=0] at (7.6,8.4) {\Large$\textcolor{color_dark_blue}{w_1}$};

    %%%%%%% Gas system %%%%%%%
    \pgfmathsetmacro{\s}{0.08}
    % Nodes
    \node[circle, fill=black, inner sep=2pt, label=below:\Large$i_{1}$] (i1) at (10,8.4) {};
    \node[circle, fill=black, inner sep=2pt, label=below:\Large$i_{2}$] (i2) at (13,8.4) {};
    \node[circle, fill=black, inner sep=2pt, label=below:\Large$i_{3}$] (i3) at (15,8.4) {};
    \node[circle, fill=black, inner sep=2pt, label=right:\Large$i_{4}$] (i4) at (13,9.4) {};
    \node[circle, fill=white, inner sep=0pt] (gfpp) at (7.2, 9.4) {};
    % Pipes
    \draw (i1) -- (i2) node[midway,below] {\Large$p_{1}$};
    \draw (i2) -- (i3) node[midway,below] {\Large$p_{2}$};
    \draw (i2) -- (i4) node[midway,left] {\Large$p_{3}$};
    % Coupling
    \draw [dashed,<->,color = color_ConvD] (i4) -- (gfpp); %(12, 9) -- (12, 10.5) -- (6.9, 10.5)
    % Gas sources
    \node[circle, draw=black, inner sep=4pt, label=left:\Large$s_{1}$] (emptyCircle) (s1) at (9.5,8.4) {};
    \draw (s1) -- (i1);
    \node[circle, draw=black, inner sep=4pt, label=right:\Large$s_{2}$] (emptyCircle) (s2) at (15.5,8.4) {};
    \draw (s2) -- (i3);
    % Gas load
    \draw[->] (i4) -- +(0,1); %l1
    \end{circuitikz}

    
